Model Checking Markov Population Models by Stochastic Approximations

Many complex systems can be described by population models, in which a pool of agents interacts and produces complex collective behaviours. We consider the problem of verifying formal properties of the underlying mathematical representation of these models, which is a Continuous Time Markov Chain, often with a huge state space. To circumvent the state space explosion, we rely on stochastic approximation techniques, which replace the large model by a simpler one, guaranteed to be probabilistically consistent. We show how to efficiently and accurately verify properties of random individual agents, specified by Continuous Stochastic Logic extended with Timed Automata (CSL-TA), and how to lift these specifications to the collective level, approximating the number of agents satisfying them using second or higher order stochastic approximation techniques.

==> background.tex <==
% !TEX root =  JournalQEST.tex


\section{Background}
\label{sec:background}

- CTMCs and piecewise CTMCs\\
- DTAs (without resets)

==> exper.tex <==
% !TEX root =  JournalQEST.tex


\section{Experimental analysis}
\label{sec:exper}

%\textit{The Epidemic Spreading.}\\
%
%\vspace{3mm}
%\noindent\textit{The Video Streaming.}
\subsection{Experimental Analysis} \label{subsec:l2g:results}
We  discuss now the quality of our method  from an experimental perspective. We present a detailed investigation of the behaviour of the running example describing a network epidemics introduced along all the paper. We consider the two local properties expressed as 1gDTAs shown in Figure \ref{DTAprop}. As said before, the first property $\gdta_1$ has no clock constraints on the edges of the automaton, therefore the 1gDTA reduces to a DFA. The property is satisfied  if an infected node is  patched before being able to infect other nodes in the network,  thus checking the effectiveness of the antivirus deployment strategy. The second property $\gdta_2$, instead, is properly timed. % and it is similar to the one of Figure \ref{DTAprop} left. 
It is satisfied  when a susceptible node is infected by an internal infection after the first $\tau$ units of time. The corresponding global properties that we consider are $\gp{\gpropg{\gdta_1(T)}{\alpha_1}}{}{}$ and $\gp{\gpropg{\gdta_2(T)}{\alpha_2}}{}{}$.

%In Figure \ref{experimentl2g}, we show the probability of the two global properties as a function of the time horizon $T$, for different values of $N$ and a specific configuration of parameters ($\kappa_{\mathit{inf}}=0.05$, $\kappa_{patch_1}=0.02$, $\kappa_{loss}=0.01$, $\kappa_{ext}=0.05$, $\kappa_{patch_0}=0.001$, $\alpha_1=0.5$, $\alpha_2=0.2$). The CLA is  compared with a statistical estimate, obtained from 10000 simulation runs.   
%As we can see, the accuracy in the transient phase increases rapidly with $N$, and  the estimate is  very good for both properties already for  $N=100$. 

In Table \ref{table:speedupl2g}, we show the computational costs (in Seconds), for
the probability of the two global properties as a function of the time horizon $T$, for different values of $N$ and a specific configuration of parameters ($\kappa_{\mathit{inf}}=0.05$, $\kappa_{patch_1}=0.02$, $\kappa_{loss}=0.01$, $\kappa_{ext}=0.05$, $\kappa_{patch_0}=0.001$, $\alpha_1=0.5$, $\alpha_2=0.2$). The CLA is  compared with a statistical estimate, obtained from 10000 simulation runs.   As we have seen, by definition the Central Limit Approximation is independent of the population size $N$ and its computational costs is hundreds of times less than that of the statistical estimate (the Gillespie Algorithm) for both the first and the second properties.  

\begin{figure}[!t]
\begin{center}
%\includegraphics[width=.47\textwidth]{figs/untimed.pdf}
%\includegraphics[width=.47\textwidth]{figs/timed.pdf}
\end{center}

\caption[Results obtained by the Central Limit Approximation and the Gillespie's Statistical Algorithm in the validation of Local-to-Global Properties.]{Comparison of Central Limit Approximation (CLA) and a statistical estimate (using the Gillespie algorithm, SSA) of the path probabilities of the 1gDTA properties of Figure \ref{DTApropExa} computed on the network epidemic model for different values of the population size $N$.}
\label{experimentl2g}
\end{figure}

\begin{table}[!t]
\begin{center}
\textbf{First Property}\\
\begin{small}
\begin{tabular}{|c||c|c|c|}
\hline
$N$ & SSAcost & CLAcost & Speedup  \\ 
\hline
    20 & 22.4114 & 0.0618 & 362.6440\\
    \hline
    50   & 23.3467  & 0.0618 & 377.7783\\
    \hline
 100   & 24.2689  & 0.0618 & 392.7006\\
 \hline
  200 &  26.1074  & 0.0618 & 442.4498\\
  \hline
  500 & 28.8754   & 0.0618 & 467.2395\\
\hline
\end{tabular}
\end{small}

\vspace{0.2cm}
\textbf{Second Property}\\
\begin{small}
\begin{tabular}{|c||c|c|c|}
\hline
$N$ & SSAcost & CLAcost & Speedup\\ 
\hline
    20 &  32.0598 & 0.3035 & 105.6336\\
    \hline
    50  & 29.0915 & 0.3035 & 95.8534\\
    \hline
 100     & 28.8651 & 0.3035 & 95.1074\\
 \hline
  200  &   33.9825 & 0.3035 & 111.9687\\
  \hline
  500   & 43.4737 & 0.3035 & 143.2412\\
\hline
\end{tabular}
\end{small}
\end{center}
\caption[Computational costs of the Central Limit Approximation in the validation of Local-to-Global Properties.]{Average computational costs (in Seconds) of the Gillespie Algorithm (SSAcost) and the Central Limit Approximation (CLAcost), and the relative SpeedUp (CLAcost/SSAcost). The data are shown as a function of the population size $N$ (by definition the CLA is independent of $N$).}
\label{table:speedupl2g}
\end{table}

In order to check extensively the quality of the approximation also as a function of the system parameters, we  ran the following experiment. We considered five different values of $N$ ($N=20,50,100,200,500$). For each of these values, we randomly chose 20 different combinations of parameter values, sampling uniformly from:  $\kappa_{\mathit{inf}} \in [0.05, 5]$, $\kappa_{patch_1} \in [0.02, 2]$, $\kappa_{loss} \in [0.01, 1]$, $\kappa_{ext} \in [0.05, 5]$, $\kappa_{patch_0} \in [0.001, 0.1]$, $\alpha_1 \in [0.1, 0.95]$, $\alpha_2 \in [0.1, 0.3]$.
For each parameter set, we compared the CLA of the probability of each global property with a statistical estimate (from 5000 runs), measuring the error in a grid of 1000 equi-spaced time points. We then computed the maximum error and the average error. In Table \ref{table:errorl2g}, we report the mean  and  maximum values of these quantities over the 20 runs, for each considered value of $N$. We also report the error at the final time of the simulation, when the probability has stabilised to its limit value.\footnote{For this model, we can extend the analysis to steady state, as the fluid limit has a unique, globally attracting steady state. This is not possible in general, cf. \cite{tutorial}.} It can be seen that both the average and the maximum errors decrease with $N$, as expected, and are already quite small for $N=100$ (for the first property, the maximum difference in the path probability for all runs is of the order of 0.06, while the average error is 0.003). For $N=500$, the CLA is practically indistinguishable from the (estimated) true probability. For the second property, the errors are slightly worse, but still reasonably small.




\begin{table}[!t]
\begin{center}
\textbf{First Property}
\begin{small}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
$N$ & MaxEr  & $\bbE$[MaxEr] & Max$\bbE$[Er] & $\bbE$[$\bbE$[Er]] & MaxEr($T$) & $\bbE$[Er($T$)] \\ 
\hline
    20  &  0.1336  &  0.0420  &  0.0491 &   0.0094  &  0.0442  &  0.0037 \\
    \hline
    50   & 0.0866   & 0.0366  &  0.0631  &  0.0067  &  0.0128   & 0.0018 \\
    \hline
 100   & 0.0611   & 0.0266   & 0.0249   & 0.0030  &  0.0307   & 0.0017 \\
 \hline
  200 & 0.0504   & 0.0191  &  0.0055   &  0.0003  &  0.0033  &  0.0002 \\
  \hline
  500 & 0.0336   & 0.0120 &   0.0024   &  0.0003 &   0.0002  &  9.5e-6 \\
\hline
\end{tabular}
\end{small}

\vspace{0.2cm}
\textbf{Second Property}
\begin{small}
\begin{tabular}{|c||c|c|c|c|c|c|}
\hline
$N$ & MaxEr  & $\bbE$[MaxEr] & Max$\bbE$[Er] & $\bbE$[$\bbE$[Er]] & MaxEr($T$) & $\bbE$[Er($T$)] \\ 
\hline
    20 &  0.2478 &    0.1173   & 0.1552 &   0.0450  &  0.1662 &   0.0448 \\
    \hline
    50  & 0.2216 &    0.0767   & 0.1233 &    0.0340 &    0.1337   & 0.0361  \\
    \hline
 100    & 0.1380   & 0.0620 &    0.0887 &    0.0216 &    0.0979 &    0.0208 \\
 \hline
  200  & 0.1365   & 0.0538 &    0.0716   & 0.0053 &    0.0779  &  0.0162 \\
  \hline
  500   & 0.1187  &  0.0398   & 0.0585   &  0.0100  &  0.0725 &    0.0108  \\
\hline
\end{tabular}
\end{small}
\end{center}
\caption[Errors obtained by the Central Limit Approximation in the validation of Local-to-Global Properties.]{Errors obtained by the Central Limit Approximation in the validation of Local-to-Global Properties. Maximum  and mean of the maximum error (MaxEr, $\bbE$[MaxEr]) for each parameter configuration;  maximum and mean of the average error with respect to time (Max$\bbE$[Er]), $\bbE$[$\bbE$[Er]])  for each parameter configuration; maximum and average error at the final time horizon $T$ (MaxEr($T$), $\bbE$[Er($T$)] ) for each parameter configuration. Data is shown as a function of the network size $N$. }
\label{table:errorl2g}
\end{table}


Finally, we considered the problem of understanding what are the most important aspects that determine the error. To this end, we regressed the observed error against the following features: estimated probability value by CLA, error in the predicted average and variance of $X_{Final}$ (between the CLA and the statistical estimates), and statistical estimates of the mean, variance, skewness and kurtosis of $X_{Final}$. We used Gaussian Process regression with Adaptive Relevance Detection (GP-ADR, \cite{gp}), which performs a regularised regression searching the best fit on an infinite dimensional subspace of continuous functions, and permitted us to identify the most relevant features by learning the hyperparameters of the kernel function. We used both a squared exponential kernel, a quadratic kernel, and a combination of the two, with a training set of 500 points, selected randomly from the experiments performed. The mean prediction error on a test set of other 500 points (independently of $N$) is around  0.015 for all the considered kernels. Furthermore, GP-ADR  selected as most relevant the quadratic kernel, and in particular the following two features: the estimated probability and the error in the mean of $X_{Final}$.  This suggests that moment closure techniques improving the prediction of the average can possibly reduce the error of the method.

\subsection{Results of System Size Expansion and Moment Closure}\label{exp:sse}
